Identifying All {\epsilon}-Best Arms in (Misspecified) Linear Bandits

Motivated by the need to efficiently identify multiple candidates in high trial-and-error cost tasks such as drug discovery, we propose a near-optimal algorithm to identify all {\epsilon}-best arms (i.e., those at most {\epsilon} worse than the optimum). Specifically, we introduce LinFACT, an algorithm designed to optimize the identification of all {\epsilon}-best arms in linear bandits. We establish a novel information-theoretic lower bound on the sample complexity of this problem and demonstrate that LinFACT achieves instance optimality by matching this lower bound up to a logarithmic factor. A key ingredient of our proof is to integrate the lower bound directly into the scaling process for upper bound derivation, determining the termination round and thus the sample complexity. We also extend our analysis to settings with model misspecification and generalized linear models. Numerical experiments, including synthetic and real drug discovery data, demonstrate that LinFACT identifies more promising candidates with reduced sample complexity, offering significant computational efficiency and accelerating early-stage exploratory experiments.

==> reference_appen.tex <==
@article{qin2025dual,
  title={Dual-directed algorithm design for efficient pure exploration},
  author={Qin, Chao and You, Wei},
  journal={Operations Research},
  year={2025},
  publisher={INFORMS}
}

@article{doi:10.1287/mnsc.2022.00328,
author = {Ahn, Dohyun and Shin, Dongwook and Zeevi, Assaf},
title = {Feature Misspecification in Sequential Learning Problems},
journal = {Management Science},
volume = {0},
number = {0},
pages = {null},
year = {2024},
doi = {10.1287/mnsc.2022.00328},

URL = { 
    
        https://doi.org/10.1287/mnsc.2022.00328
    
    

},
eprint = { 
    
        https://doi.org/10.1287/mnsc.2022.00328
    
    

}
,
    abstract = { We consider a class of sequential learning problems where a decision maker must learn the unknown statistical characteristics of a finite set of alternatives (or systems) using sequential sampling to ultimately select a subset of “good” alternatives. A salient feature of our problem is that system performance is governed by a set of features. The decision maker postulates the dependence on these features to be linear, but this model may not precisely represent the true underlying system structure. We show that this misspecification, if not managed properly, can lead to suboptimal performance because of a phenomenon identified as sample-selection endogeneity. We propose a prospective sampling principle—a new approach that eliminates the adverse effects of misspecification as the number of samples grows large. The proposed principle applies across a very general class of widely used sampling policies, enjoys strong asymptotic performance guarantees, and exhibits effective finite-sample performance in numerical experiments.This paper was accepted by Vivek Farias, data science.Funding: This work was supported by the United States-Israel Binational Science Foundation [Grant 2020063] and the Hong Kong Research Grant Council [GRF Grant 16501821 and ECS Grant 24210420].Supplemental Material: The online appendix and data files are available at https://doi.org/10.1287/mnsc.2022.00328. }
}

@article{feng2022robust,
  title={Robust learning of consumer preferences},
  author={Feng, Yifan and Caldentey, Ren{\'e} and Ryan, Christopher Thomas},
  journal={Operations Research},
  volume={70},
  number={2},
  pages={918--962},
  year={2022},
  publisher={INFORMS}
}

@inproceedings{yang2023nested,
  title={Nested elimination: a simple algorithm for best-item identification from choice-based feedback},
  author={Yang, Junwen and Feng, Yifan},
  booktitle={International Conference on Machine Learning},
  pages={39205--39233},
  year={2023},
  organization={PMLR}
}

@inproceedings{ahn2020ordinal,
  title={Ordinal optimization with generalized linear model},
  author={Ahn, Dohyun and Shin, Dongwook},
  booktitle={2020 Winter Simulation Conference (WSC)},
  pages={3008--3019},
  year={2020},
  organization={IEEE}
}

@article{shen2021ranking,
  title={Ranking and selection with covariates for personalized decision making},
  author={Shen, Haihui and Hong, L Jeff and Zhang, Xiaowei},
  journal={INFORMS Journal on Computing},
  volume={33},
  number={4},
  pages={1500--1519},
  year={2021},
  publisher={INFORMS}
}

@article{shin2018tractable,
  title={Tractable sampling strategies for ordinal optimization},
  author={Shin, Dongwook and Broadie, Mark and Zeevi, Assaf},
  journal={Operations Research},
  volume={66},
  number={6},
  pages={1693--1712},
  year={2018},
  publisher={INFORMS}
}

@article{ahn2023feature,
  title={Feature Misspecification in Sequential Learning Problems},
  author={Ahn, Dohyun and Shin, Dongwook and Zeevi, Assaf},
  journal={Columbia Business School Research Paper},
  year={2023}
}

@article{huang2007analyzing,
  title={Analyzing consumer-product graphs: Empirical findings and applications in recommender systems},
  author={Huang, Zan and Zeng, Daniel D and Chen, Hsinchun},
  journal={Management science},
  volume={53},
  number={7},
  pages={1146--1164},
  year={2007},
  publisher={INFORMS}
}

@article{peukert2023editor,
  title={The editor and the algorithm: Recommendation technology in online news},
  author={Peukert, Christian and Sen, Ananya and Claussen, J{\"o}rg},
  journal={Management science},
  year={2023},
  publisher={INFORMS}
}

@inproceedings{zanette2020learning,
  title={Learning near optimal policies with low inherent bellman error},
  author={Zanette, Andrea and Lazaric, Alessandro and Kochenderfer, Mykel and Brunskill, Emma},
  booktitle={International Conference on Machine Learning},
  pages={10978--10989},
  year={2020},
  organization={PMLR}
}

@article{russo2018tutorial,
  title={A tutorial on thompson sampling},
  author={Russo, Daniel J and Van Roy, Benjamin and Kazerouni, Abbas and Osband, Ian and Wen, Zheng and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={11},
  number={1},
  pages={1--96},
  year={2018},
  publisher={Now Publishers, Inc.}
}

@article{chapelle2011empirical,
  title={An empirical evaluation of thompson sampling},
  author={Chapelle, Olivier and Li, Lihong},
  journal={Advances in neural information processing systems},
  volume={24},
  year={2011}
}

@inproceedings{10.1145/1772690.1772758,
author = {Li, Lihong and Chu, Wei and Langford, John and Schapire, Robert E.},
title = {A contextual-bandit approach to personalized news article recommendation},
year = {2010},
isbn = {9781605587998},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1772690.1772758},
doi = {10.1145/1772690.1772758},
abstract = {Personalized web services strive to adapt their services (advertisements, news articles, etc.) to individual users by making use of both content and user information. Despite a few recent advances, this problem remains challenging for at least two reasons. First, web service is featured with dynamically changing pools of content, rendering traditional collaborative filtering methods inapplicable. Second, the scale of most web services of practical interest calls for solutions that are both fast in learning and computation.In this work, we model personalized recommendation of news articles as a contextual bandit problem, a principled approach in which a learning algorithm sequentially selects articles to serve users based on contextual information about the users and articles, while simultaneously adapting its article-selection strategy based on user-click feedback to maximize total user clicks.The contributions of this work are three-fold. First, we propose a new, general contextual bandit algorithm that is computationally efficient and well motivated from learning theory. Second, we argue that any bandit algorithm can be reliably evaluated offline using previously recorded random traffic. Finally, using this offline evaluation method, we successfully applied our new algorithm to a Yahoo! Front Page Today Module dataset containing over 33 million events. Results showed a 12.5\% click lift compared to a standard context-free bandit algorithm, and the advantage becomes even greater when data gets more scarce.},
booktitle = {Proceedings of the 19th International Conference on World Wide Web},
pages = {661–670},
numpages = {10},
keywords = {contextual bandit, exploration/exploitation dilemma, personalization, recommender systems, web service},
location = {Raleigh, North Carolina, USA},
series = {WWW '10}
}

@article{ryzhov2012knowledge,
  title={The knowledge gradient algorithm for a general class of online learning problems},
  author={Ryzhov, Ilya O and Powell, Warren B and Frazier, Peter I},
  journal={Operations Research},
  volume={60},
  number={1},
  pages={180--195},
  year={2012},
  publisher={INFORMS}
}

@article{frazier2009knowledge,
  title={The knowledge-gradient policy for correlated normal beliefs},
  author={Frazier, Peter and Powell, Warren and Dayanik, Savas},
  journal={INFORMS journal on Computing},
  volume={21},
  number={4},
  pages={599--613},
  year={2009},
  publisher={INFORMS}
}

@inproceedings{thornton2013auto,
  title={Auto-WEKA: Combined selection and hyperparameter optimization of classification algorithms},
  author={Thornton, Chris and Hutter, Frank and Hoos, Holger H and Leyton-Brown, Kevin},
  booktitle={Proceedings of the 19th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={847--855},
  year={2013}
}

@article{bastani2021predicting,
  title={Predicting with proxies: Transfer learning in high dimension},
  author={Bastani, Hamsa},
  journal={Management Science},
  volume={67},
  number={5},
  pages={2964--2984},
  year={2021},
  publisher={INFORMS}
}

@article{boyd2003revenue,
  title={Revenue management and e-commerce},
  author={Boyd, E Andrew and Bilegan, Ioana C},
  journal={Management science},
  volume={49},
  number={10},
  pages={1363--1386},
  year={2003},
  publisher={INFORMS}
}

@article{doi:10.1287/mnsc.1050.0427,
author = {Song, Jaeki and Zahedi, Fatemeh “Mariam”},
title = {A Theoretical Approach to Web Design in E-Commerce: A Belief Reinforcement Model},
journal = {Management Science},
volume = {51},
number = {8},
pages = {1219-1235},
year = {2005},
doi = {10.1287/mnsc.1050.0427},

URL = { 
    
        https://doi.org/10.1287/mnsc.1050.0427
    
    

},
eprint = { 
    
        https://doi.org/10.1287/mnsc.1050.0427
    
    

}
,
    abstract = { Effective website design plays a critical role in attracting and maintaining customers’ interest. Despite the importance of websites as the major and, at times, sole channel of communication in e-business, little theoretical knowledge is available about how websites may influence online shoppers’ attitudes and behavior. In this paper, we develop a conceptual framework for measuring the impact of Web-design elements on the beliefs and behavior of Web customers. In developing the theoretical model (called the belief reinforcement model, or BRM), we synthesize the theory of planned behavior with theories in social psychology, consumer behavior, and management to categorize Web-design elements and conceptualize the salient aspects of Web shoppers’ behavior. The empirical examination of BRM indicates that various categories of Web-design elements reinforce Web customers’ beliefs, which in turn positively impact attitudinal constructs that lead to changes in their purchase intentions. BRM and its results provide an initial guideline for a rigorous approach to designing websites for e-business and testing their effectiveness before their full deployment. }
}

@article{banker200450th,
  title={50th anniversary article: The evolution of research on information systems: A fiftieth-year survey of the literature in management science},
  author={Banker, Rajiv D and Kauffman, Robert J},
  journal={Management science},
  volume={50},
  number={3},
  pages={281--298},
  year={2004},
  publisher={INFORMS}
}

@article{doi:10.1287/mnsc.2022.4307,
author = {Alaei, Saeed and Makhdoumi, Ali and Malekian, Azarakhsh and Peke\v{c}, Sa\v{s}a},
title = {Revenue-Sharing Allocation Strategies for Two-Sided Media Platforms: Pro-Rata vs. User-Centric},
journal = {Management Science},
volume = {68},
number = {12},
pages = {8699-8721},
year = {2022},
doi = {10.1287/mnsc.2022.4307},

URL = { 
    
        https://doi.org/10.1287/mnsc.2022.4307
    
    

},
eprint = { 
    
        https://doi.org/10.1287/mnsc.2022.4307
    
    

}
,
    abstract = { We consider a two-sided streaming service platform that generates revenues by charging users a subscription fee for unlimited access to the content and compensates content providers (artists) through a revenue-sharing allocation rule. Platform users are heterogeneous in both their overall consumption and the distribution of their consumption over different artists. We study two primary revenue allocation rules used by market-leading music streaming platforms—pro-rata and user-centric. With pro-rata, artists are paid proportionally to their share of the overall streaming volume, whereas with user-centric, each user’s subscription fee is divided proportionally among artists based on the consumption of that user. We characterize when these two allocation rules can sustain a set of artists on the platform and compare them from both the platform’s and the artists’ perspectives. In particular, we show that, despite the cross-subsidization between low- and high-streaming-volume users, the pro-rata rule can be preferred by both the platform and the artists. Furthermore, the platform’s problem of selecting an optimal portfolio of artists is NP-complete. However, by establishing connections to the knapsack problem, we develop a polynomial time approximation scheme (PTAS) for the optimal platform’s profit. In addition to determining the platform’s optimal revenue allocation rule in the class of pro-rata and user-centric rules, we consider the optimal revenue allocation rule in the class of arbitrary rules. Building on duality theory, we develop a polynomial time algorithm that outputs a set of artists so that the platform’s profit is within a single artist’s revenue from the optimal profit.This paper was accepted by Gabriel Weintraub, revenue management and market analytics.Supplemental Material: The online appendices are available at https://doi.org/10.1287/mnsc.2022.4307. }
}

@article{doi:10.1287/mnsc.2017.2875,
author = {Godinho de Matos, Miguel and Ferreira, Pedro and Smith, Michael D.},
title = {The Effect of Subscription Video-on-Demand on Piracy: Evidence from a Household-Level Randomized Experiment},
journal = {Management Science},
volume = {64},
number = {12},
pages = {5610-5630},
year = {2018},
doi = {10.1287/mnsc.2017.2875},

URL = { 
    
        https://doi.org/10.1287/mnsc.2017.2875
    
    

},
eprint = { 
    
        https://doi.org/10.1287/mnsc.2017.2875
    
    

}
,
    abstract = { We partner with a major multinational telecommunications provider to analyze the effect of subscription video-on-demand (SVoD) services on digital piracy. For a period of 45 consecutive days, a group of randomly selected households who used BitTorrent in the past were gifted with a bundle of TV channels with movies and TV shows that could be streamed as in SVoD. We find that, on average, households that received the gift increased overall TV consumption by 4.6\% and reduced Internet downloads and uploads by 4.2\% and 4.5\%, respectively. However, and also on average, treated households did not change their likelihood of using BitTorrent during the experiment. Our findings are heterogeneous across households and are mediated by the fit between the preferences of households in our sample for movies and the content available as part of the gifted channels. Households with preferences aligned with the gifted content reduced their probability of using BitTorrent during the experiment by 18\% and decreased their amount of upload traffic by 45\%. We also show using simulation that the size of the SVoD catalog and licensing window restrictions limit significantly the ability of content providers to match SVoD offerings to the preferences of BitTorrent users. Finally, we estimate that households in our sample are willing to pay at most \$3.25 USD per month to access a SVoD catalog as large as Netflix’s in the United States. Together, our results show that, as a stand-alone strategy, using legal SVoD to curtail piracy will require, at the minimum, offering content much earlier and at much lower prices than those currently offered in the marketplace, changes that are likely to reduce industry revenue and that may damage overall incentives to produce new content while, at the same time, curbing only a small share of piracy. The online appendix is available at https://doi.org/10.1287/mnsc.2017.2875. This paper was accepted by Chris Forman, information systems. }
}


@article{elmaghraby2003dynamic,
  title={Dynamic pricing in the presence of inventory considerations: Research overview, current practices, and future directions},
  author={Elmaghraby, Wedad and Keskinocak, P{\i}nar},
  journal={Management science},
  volume={49},
  number={10},
  pages={1287--1309},
  year={2003},
  publisher={INFORMS}
}

@article{komiyama2023rate,
  title={Rate-optimal bayesian simple regret in best arm identification},
  author={Komiyama, Junpei and Ariu, Kaito and Kato, Masahiro and Qin, Chao},
  journal={Mathematics of Operations Research},
  year={2023},
  publisher={INFORMS}
}

@article{doi:10.1287/opre.2019.1911,
author = {Russo, Daniel},
title = {Simple Bayesian Algorithms for Best-Arm Identification},
journal = {Operations Research},
volume = {68},
number = {6},
pages = {1625-1647},
year = {2020},
doi = {10.1287/opre.2019.1911},

URL = { 
    
        https://doi.org/10.1287/opre.2019.1911
    
    

},
eprint = { 
    
        https://doi.org/10.1287/opre.2019.1911
    
    

}
,
    abstract = { This paper considers the optimal adaptive allocation of measurement effort for identifying the best among a finite set of options or designs. An experimenter sequentially chooses designs to measure and observes noisy signals of their quality with the goal of confidently identifying the best design after a small number of measurements. Just as the multiarmed bandit problem crystallizes the tradeoff between exploration and exploitation, this “pure exploration” variant crystallizes the challenge of rapidly gathering information before committing to a final decision. The paper proposes several simple Bayesian algorithms for allocating measurement effort and, by characterizing fundamental asymptotic limits on the performance of any algorithm, formalizes a sense in which these seemingly naive algorithms are the best possible. }
}

@inproceedings{russo2016simple,
  title={Simple bayesian algorithms for best arm identification},
  author={Russo, Daniel},
  booktitle={Conference on Learning Theory},
  pages={1417--1418},
  year={2016},
  organization={PMLR}
}

@article{li2024surprising,
  title={The (Surprising) Sample Optimality of Greedy Procedures for Large-Scale Ranking and Selection},
  author={Li, Zaile and Fan, Weiwei and Hong, L Jeff},
  journal={Management Science},
  year={2024},
  publisher={INFORMS}
}

@inproceedings{hunter2017parallel,
  title={Parallel ranking and selection},
  author={Hunter, Susan R and Nelson, Barry L},
  booktitle={Advances in Modeling and Simulation: Seminal Research from 50 Years of Winter Simulation Conferences},
  pages={249--275},
  year={2017},
  organization={Springer}
}

@article{kim2006selecting,
  title={Selecting the best system},
  author={Kim, Seong-Hee and Nelson, Barry L},
  journal={Handbooks in operations research and management science},
  volume={13},
  pages={501--534},
  year={2006},
  publisher={Elsevier}
}
